An Intuitive Automated Modelling Interface for Systems Biology

We introduce a natural language interface for building stochastic pi calculus models of biological systems. In this language, complex constructs describing biochemical events are built from basic primitives of association, dissociation and transformation. This language thus allows us to model biochemical systems modularly by describing their dynamics in a narrative-style language, while making amendments, refinements and extensions on the models easy. We demonstrate the language on a model of Fc-gamma receptor phosphorylation during phagocytosis. We provide a tool implementation of the translation into a stochastic pi calculus language, Microsoft Research's SPiM.

==> eptcsdata.tex <==
\providecommand{\event}{S. Barry Cooper \& Vincent Danos (eds.): Fifth Workshop on\\
Developments in Computational Models---Computational Models From Nature}
\providecommand{\volume}{9}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{73}
\providecommand{\eid}{9}
\pdfoutput=1

